Risk-Sensitive Deep RL: Variance-Constrained Actor-Critic Provably Finds Globally Optimal Policy

While deep reinforcement learning has achieved tremendous successes in various applications, most existing works only focus on maximizing the expected value of total return and thus ignore its inherent stochasticity. Such stochasticity is also known as the aleatoric uncertainty and is closely related to the notion of risk. In this work, we make the first attempt to study risk-sensitive deep reinforcement learning under the average reward setting with the variance risk criteria. In particular, we focus on a variance-constrained policy optimization problem where the goal is to find a policy that maximizes the expected value of the long-run average reward, subject to a constraint that the long-run variance of the average reward is upper bounded by a threshold. Utilizing Lagrangian and Fenchel dualities, we transform the original problem into an unconstrained saddle-point policy optimization problem, and propose an actor-critic algorithm that iteratively and efficiently updates the policy, the Lagrange multiplier, and the Fenchel dual variable. When both the value and policy functions are represented by multi-layer overparameterized neural networks, we prove that our actor-critic algorithm generates a sequence of policies that finds a globally optimal policy at a sublinear rate. Further, We provide numerical studies of the proposed method using two real datasets to back up the theoretical results.

==> sketch.tex <==
\section{Proof Sketch}\label{sec:sketch}
In this section, we sketch the proof of Theorem \ref{thm:main}. In detail, we cast VARAC in Algorithm \ref{alg:risac} as infinite-dimensional mirror descent with primal and dual errors and show the approximation to the saddle point to establish its global convergence.

Recall that the objective $\cL(\pi)$ is defined in \eqref{eq:def-L} and $\nu^*$ is the stationary state distribution of the optimal policy $\pi^*$. 
\begin{lemma}[Performance Difference]\label{lem:v-diff}
For $\cL(\lambda, \pi, y)$ defined in \eqref{eq:def-L}, we have
\$
\cL(\lambda, \pi^*, y) - \cL(\lambda, \pi, y) = \EE_{\nu^*}[\la (1 + 2\lambda y)Q^{\pi}(s,\cdot) - \lambda W^{\pi}(s, \cdot), \pi^*(\cdot\,|\,s) - \pi(\cdot\,|\,s)\ra].
\$
\end{lemma}
\begin{proof} See Appendix \ref{appendix:proof-sketch} for a detailed proof.\end{proof}

 

\begin{lemma}[One-Step Descent of $\lambda$]\label{lem:main-descent-lambda}
	For the optimal solution $\lambda^*$ and $\overline{\lambda}_k$ obtained in \eqref{eq:update-lambda-form}, we have 
\#\label{eq:descent-lambda}
&\| \lambda^* - \overline{\lambda}_k\|^2 - \|\lambda^* - \overline{\lambda}_{k+1} \|^2   \\
&\quad\geq -\frac{1}{\gamma_k} \cdot (\cL(\lambda^*, \pi_{\theta_k},\overline{y}_k) - \cL(\overline{\lambda}_k, \pi_{\theta_k},\overline{y}_k) )  - \frac{1}{\gamma_k}\cdot2N\cdot(d_k + 2Mc_k)  \notag\\
&\quad\qquad - \frac{1}{4\gamma_k^2}\cdot(\alpha+ F +  3M^2 + 2Mc_k + d_k)^2. \notag
\#
\end{lemma}
\begin{proof}
	See Appendix \ref{appendix:proof-sketch} for a detailed proof.
\end{proof}

\begin{lemma}[One-Step Descent of $\pi$]\label{lem:main-descent}
	For the ideal improved policy $\pi_{k+1}$ defined in \eqref{eq:pi-new-true} and the current policy $\pi_{\theta_{k}}$, we have that, for any $s \in \cS$,
	\$
	&{\rm KL}(\pi^*(\cdot\,|\,s)\,\|\,\pi_{\theta_{k+1}}(\cdot\,|\,s)) - {\rm KL}(\pi^*(\cdot\,|\,s)\,\|\,\pi_{\theta_{k}}(\cdot\,|\,s))\\
	& \quad\leq \la \log(\pi_{\theta_{k+1}}(\cdot\,|\,s)/\pi_{k+1}(\cdot\,|\,s)), \pi_{\theta_k}(\cdot\,|\,s)-\pi^*(\cdot\,|\,s) \ra \\
	&\quad\qquad- \beta_k^{-1}\cdot\la(1+2y^*\overline{\lambda}_k)Q^{\pi_{\theta_k}}(s, \cdot) - \overline{\lambda}_kW^{\pi_{\theta_k}}(s, \cdot), \pi^*(\cdot\,|\,s) - \pi_{\theta_{k}}(\cdot\,|\,s)\ra\notag\\
	&\quad\qquad + \beta_k^{-1}\cdot\la(2(y^* - \overline{y}_k)\overline{\lambda}_k)Q^{\pi_{\theta_k}}(s, \cdot), \pi^*(\cdot\,|\,s) - \pi_{\theta_{k}}(\cdot\,|\,s)\ra\notag\\
	&\quad\qquad - \la \tau_{k+1}^{-1}f_{\theta_{k+1}}(s, \cdot) - \tau_k^{-1}f_{\theta_k}(s, \cdot), \pi_{\theta_{k}}(\cdot\,|\,s) - \pi_{\theta_{k+1}}(\cdot\,|\,s) \ra - 1/2\cdot\|\pi_{\theta_{k+1}}(\cdot\,|\,s) - \pi_{\theta_{k}}(\cdot\,|\,s)\|_1^2.
	\$
\end{lemma}
\begin{proof}
	See Appendix \ref{appendix:proof-sketch} for a detailed proof.
\end{proof}





\begin{lemma}[One-Step Descent of $y$]\label{lem:main-descent-y}
	For the optimal solution $y^*$ and $\overline{y}_k$ obtained in \eqref{eq:update-y-form}, we have 
	\$
	\cL(\overline{\lambda}_k, \pi_{\theta_k}, y^*) - \cL(\overline{\lambda}_k, \pi_{\theta_k}, \overline{y}_k)  \le 4MNc_k.
	\$
\end{lemma}
\begin{proof}
	See Appendix \ref{appendix:proof-sketch} for a detailed proof.
\end{proof}






Based on Lemmas \ref{lem:v-diff}, \ref{lem:main-descent-lambda}, \ref{lem:main-descent} and \ref{lem:main-descent-y}, we prove Theorem \ref{thm:main} by casting VARAC as infinite-dimensional mirror descent with primal and dual errors.


\begin{proof}[Proof of Theorem \ref{thm:main}] 
We show convergence in two parts. \\
\noindent\textbf{Part 1.}
%By telescoping \eqref{eq:descent-lambda} for $k+1\in [K]$, we obtain 
%\# \label{eq:lambda111}
%&\frac{1}{K}\sum_{k=0}^{K-1} ( (\cL(\lambda^*, \pi_{\theta_k},\overline{y}_k) - \cL(\overline{\lambda}_k, \pi_{\theta_k},\overline{y}_k)) \\
%&\quad \geq\frac{\|\lambda^* - \overline{\lambda}_K\|^2 - \|\lambda^* - \overline{\lambda}_0\|^2 - \sum_{k=0}^{K-1}\gamma_k^{-1}\cdot2N\cdot(d_k + 2Mc_k)   }{\sum_{k=0}^{K-1}\gamma_k^{-1}}     \notag\\
%&\quad\qquad - \frac{\sum_{k=0}^{K-1}\gamma_k^{-2}(\alpha+ F + 3M^2 + 2Mc_k + d_k)^2 }{4\sum_{k=0}^{K-1}\gamma_k^{-1}} .\notag
%\#
Setting the parameter $\gamma_k =\gamma\sqrt{K}$ and telescoping \eqref{eq:descent-lambda} for $k+1\in [K]$, we have
\#\label{eq:result-part1}
&\frac{1}{K}\sum_{k=0}^{K-1} ( (\cL(\lambda^*, \pi_{\theta_k},\overline{y}_k) - \cL(\overline{\lambda}_k, \pi_{\theta_k},\overline{y}_k)) \\
&\quad\geq \frac{\|\lambda^* - \overline{\lambda}_K\|^2 - \|\lambda^* - \overline{\lambda}_0\|^2 - 2N\sum_{k=0}^{K-1} (d_k + 2Mc_k)}{K}  - \frac{\sum_{k=0}^{K-1}(\alpha+ F + 3M^2 + 2Mc_k + d_k)^2  }{4\gamma K \sqrt{K}} \notag \\
&\quad = - \sum_{k=0}^{K-1} (c_k + d_k)^2\cdot O(1/K\sqrt{K}) - \sum_{k=0}^{K-1} (c_k + d_k)\cdot O(1/K)  - O(1/K).\notag
\#
Using saddle-point relation that $\cL(\lambda^*, \pi_{\theta_k},\overline{y}_k) \leq \cL(\lambda^*, \pi^*, y^*) $, we complete the proof of the first part of Theorem \ref{thm:main}. 






\vskip5pt
\noindent\textbf{Part 2.}
Taking expectation with respect to $s\sim\nu^*$ and invoking Lemmas \ref{lem:error-kl} and \ref{lem:main-descent}, we have
\$
&\EE_{\nu^*}[{\rm KL}(\pi^*(\cdot\,|\,s)\,\|\,\pi_{\theta_{k+1}}(\cdot\,|\,s))] - \EE_{\nu^*}[{\rm KL}(\pi^*(\cdot\,|\,s)\,\|\,\pi_{\theta_{k}}(\cdot\,|\,s))] \notag\\
&\quad\le
\varepsilon_{k} - \beta_k^{-1}\cdot \EE_{\nu^*}[\la(1+2y^*\overline{\lambda}_k)Q^{\pi_{\theta_k}}(s, \cdot) - \overline{\lambda}_kW^{\pi_{\theta_k}}(s, \cdot), \pi^*(\cdot\,|\,s) - \pi_{\theta_{k}}(\cdot\,|\,s)\ra] \notag\\
%&\quad\qquad \EE_{\nu^*}[\la(2(\overline{y}_k - y^*)\overline{\lambda}_k)Q^{\pi_{\theta_k}}(s, \cdot), \pi^*(\cdot\,|\,s) - \pi_{\theta_{k}}(\cdot\,|\,s)\ra] \norag\\
&\quad\qquad + \beta_k^{-1}\cdot \EE_{\nu^*}[\la2(y^*-\overline{y}_k)\overline{\lambda}_kQ^{\pi_{\theta_k}}(s, \cdot), \pi^*(\cdot\,|\,s) - \pi_{\theta_{k}}(\cdot\,|\,s)\ra] \notag\\
&\quad\qquad
- \EE_{\nu^*}[\la \tau_{k+1}^{-1}f_{\theta_{k+1}}(s, \cdot) - \tau_k^{-1}f_{\theta_k}(s, \cdot),  \pi_{\theta_k}(\cdot\,|\,s)- \pi_{\theta_{k+1}}(\cdot\,|\,s)  \ra] \notag\\
&\quad\qquad - 1/2\cdot\EE_{\nu^*}[ \|\pi_{\theta_{k+1}}(\cdot\,|\,s) - \pi_{\theta_{k}}(\cdot\,|\,s)\|^2_1 ].
\$
By Lemma \ref{lem:v-diff} and the H{\"o}lder's inequality, we further have
\#\label{812209}
&\EE_{\nu^*}[{\rm KL}(\pi^*(\cdot\,|\,s)\,\|\,\pi_{\theta_{k+1}}(\cdot\,|\,s))] - \EE_{\nu^*}[{\rm KL}(\pi^*(\cdot\,|\,s)\,\|\,\pi_{\theta_{k}}(\cdot\,|\,s))] \notag\\
&\quad\le
\varepsilon_{k} - \beta_k^{-1}\cdot(\cL(\overline{\lambda}_k,\pi^*, y^*) - \cL(\overline{\lambda}_k,\pi_{\theta_k}, y^*))   +\beta_k^{-1}\cdot(2\overline{\lambda}_k(\overline{y}_k-y^*))\cdot(\rho(\pi^*) - \rho(\pi_{\theta{k}}))  \notag\\
&\quad\qquad  +\EE_{\nu^*}[\| \tau_{k+1}^{-1}f_{\theta_{k+1}}(s,\cdot)- \tau_{k}^{-1}f_{\theta_{k}}(s,\cdot)\|_{\infty}\cdot \|  \pi_{\theta_k}(\cdot\,|\,s)- \pi_{\theta_{k+1}}(\cdot\,|\,s) \|_1]\notag\\
&\quad\qquad - 1/2\cdot\EE_{\nu^*}[ \|\pi_{\theta_{k+1}}(\cdot\,|\,s) - \pi_{\theta_{k}}(\cdot\,|\,s)\|^2_1 ] \notag\\
&\quad\le
\varepsilon_{k} - \beta_k^{-1}\cdot(\cL(\overline{\lambda}_k,\pi^*, y^*) - \cL(\overline{\lambda}_k,\pi_{\theta_k}, y^*))   +\beta_k^{-1}\cdot(2\overline{\lambda}_k(\overline{y}_k-y^*))\cdot(\rho(\pi^*) - \rho(\pi_{\theta{k}}))  \notag\\
&\quad\qquad + 1/2 \cdot \EE_{\nu^*}[ \| \tau_{k+1}^{-1}f_{\theta_{k+1}}(s,\cdot)- \tau_{k}^{-1}f_{\theta_{k}}(s,\cdot)\|_{\infty}^2 ]\notag\\
&\quad\le
\varepsilon_{k} - \beta_k^{-1}\cdot(\cL(\overline{\lambda}_k,\pi^*, y^*) - \cL(\overline{\lambda}_k,\pi_{\theta_k}, y^*))   \notag\\
&\quad\qquad +\beta_k^{-1}\cdot(2\overline{\lambda}_k(\overline{y}_k-y^*))\cdot(\rho(\pi^*) - \rho(\pi_{\theta{k}})) + (\varepsilon_k'+\beta_k^{-2}\hat{M}), \#
where in the second inequality we use $2xy - y^2 \leq x^2$ and in the last inequality we use  Lemma \ref{lem:stepwise-energy}. Rearranging the terms in \eqref{812209}, we have
\#\label{812334}
&\beta_k^{-1}\cdot \bigl(\cL(\overline{\lambda}_k,\pi^*, y^*) - \cL(\overline{\lambda}_k,\pi_{\theta_k}, y^*)\bigr) \\
&\quad \le 
\EE_{\nu^*}[{\rm KL}(\pi^*(\cdot\,|\,s)\,\|\,\pi_{\theta_{k}}(\cdot\,|\,s))] - \EE_{\nu^*}[{\rm KL}(\pi^*(\cdot\,|\,s)\,\|\,\pi_{\theta_{k+1}}(\cdot\,|\,s))] \notag\\
&\quad\qquad + 2\beta_k^{-1}\cdot\overline{\lambda}_k(\overline{y}_k-y^*)\cdot(\rho(\pi^*) - \rho(\pi_{\theta{k}}))
+\beta_k^{-2} \hat{M} + \varepsilon_k + \varepsilon_k'.\notag
\#
Recall Lemma \ref{lem:main-descent-y}, we have
\#\label{eq:812335}
\cL(\overline{\lambda}_k, \pi_{\theta_k}, y^*) - \cL(\overline{\lambda}_k, \pi_{\theta_k}, \overline{y}_k)  \le 4MNc_k .
\#
And by the rule of updating $y$ and the fact that $y^*=\rho(\pi^*)$ we have 
\#\label{eq:812444}
&\overline{\lambda}_k(\overline{y}_k-y^*)\cdot(\rho(\pi^*) - \rho(\pi_{\theta{k}}))  \\
&\quad=\overline{\lambda}_k [  (\overline{y}_k-y^*)\cdot(  \overline{\rho}(\pi_{\theta{k}})- \rho(\pi_{\theta{k}}))
 +(\overline{y}_k-\overline{\rho}(\pi_{\theta_k}))\cdot(\rho(\pi^*) - \overline{\rho}(\pi_{\theta{k}}))
 -(\rho(\pi^*) - \overline{\rho}(\pi_{\theta{k}}))^2   ]  \notag \\ 
&\quad \le N\cdot(2Mc_k + 2Mc_k)  \notag\\
&\quad = 4MNc_k, \notag 
\# 
where the inequality is obtained by Assumption \ref{assumption:bounded-reward} and the fact that $  \overline{\lambda}_k(\overline{y}_k-y^*)^2$ is nonnegative.
Plugging \eqref{eq:812444} and \eqref{eq:812335} into \eqref{812334}, we obtain
\#\label{eq:812336}
&\beta_k^{-1}\cdot \bigl(\cL(\overline{\lambda}_k,\pi^*, y^*) - \cL(\overline{\lambda}_k,\pi_{\theta_k}, \overline{y}_k)\bigr) \\
&\quad \le 
\EE_{\nu^*}[{\rm KL}(\pi^*(\cdot\,|\,s)\,\|\,\pi_{\theta_{k}}(\cdot\,|\,s))] - \EE_{\nu^*}[{\rm KL}(\pi^*(\cdot\,|\,s)\,\|\,\pi_{\theta_{k+1}}(\cdot\,|\,s))] \notag\\
&\quad\qquad +\beta_k^{-2} \hat{M} +\beta_k^{-1}\cdot8MNc_k+ \varepsilon_k + \varepsilon_k'.  \notag
\#
By telescoping \eqref{eq:812336} for $k+1\in [K]$, we obtain
\$
&\sum_{k=0}^{K-1} \beta_k^{-1}\cdot(\cL(\overline{\lambda}_k,\pi^*, y^*) - \cL(\overline{\lambda}_k, \pi_{\theta_k}, \overline{y}_k))\notag\\
&\quad \le 
 \EE_{\nu^*}[{\rm KL}(\pi^*(\cdot\,|\,s)\,\|\,\pi_{\theta_{0}}(\cdot\,|\,s))] - \EE_{\nu^*}[{\rm KL}(\pi^*(\cdot\,|\,s)\,\|\,\pi_{\theta_{K}}(\cdot\,|\,s))] \notag\\
&\quad\qquad + \sum_{k=0}^{K-1}(\beta_k^{-2} \hat{M} +\beta_k^{-1}\cdot8MNc_k+ \varepsilon_k + \varepsilon_k')  .
\$
Note that we have (i) $\EE_{\nu^*}[{\rm KL}(\pi^*(\cdot\,|\,s)\,\|\,\pi_{\theta_0}(\cdot\,|\,s))] \leq \log|\cA|$ due to the uniform initialization of policy, and that (ii) the KL-divergence is nonnegative. Setting the parameter $\beta_k = \beta\sqrt{K},$  we have
\# \label{eq:result-part2}
&\frac{1}{K}\sum_{k=0}^{K-1} (\cL(\overline{\lambda}_k,\pi^*, y^*) - \cL(\overline{\lambda}_k, \pi_{\theta_k}, \overline{y}_k)) \\
 &\quad\le \frac{8MN\sum_{k=0}^{K-1}c_k}{K} +
 \frac{\beta\log|\cA| +  \beta^{-1} \hat{M} +\sum_{k=0}^{K-1}(  \varepsilon_k + \varepsilon_k')}{\sqrt{K}}  \notag\\
 &\quad   =\sum_{k=0}^{K-1}c_k \cdot O(1/K) +   \sum_{k=0}^{K-1}(  \varepsilon_k + \varepsilon_k') \cdot  O(1/\sqrt{K}) + O(1\sqrt{K})  \notag                 .
\#
Using saddle-point relation that $\cL(\overline{\lambda}_k,\pi^*, y^*) \geq \cL(\lambda^*, \pi^*, y^*) $, we finish the proof of the second part of Theorem \ref{thm:main}.
\end{proof}

